Crafting Adversarial Examples For Speech Paralinguistics Applications

Computational paralinguistic analysis is increasingly being used in a wide range of cyber applications, including security-sensitive applications such as speaker verification, deceptive speech detection, and medical diagnostics. While state-of-the-art machine learning techniques, such as deep neural networks, can provide robust and accurate speech analysis, they are susceptible to adversarial attacks. In this work, we propose an end-to-end scheme to generate adversarial examples for computational paralinguistic applications by perturbing directly the raw waveform of an audio recording rather than specific acoustic features. Our experiments show that the proposed adversarial perturbation can lead to a significant performance drop of state-of-the-art deep neural networks, while only minimally impairing the audio quality.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	samples/sample-manuscript.tex \
	samples/sample-acmsmall.tex \
	samples/sample-acmlarge.tex \
	samples/sample-acmtog.tex \
	samples/sample-sigconf.tex \
	samples/sample-authordraft.tex \
	samples/sample-xelatex.tex \
	samples/sample-sigplan.tex \
	samples/sample-sigchi.tex \
	samples/sample-sigchi-a.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

samples/%: %
	cp $^ samples

samples/sample-acmsmall.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmsmall]{acmart}/' $< > $@

samples/sample-acmlarge.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmlarge,screen]{acmart}/' $< > $@

samples/sample-acmtog.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmtog]{acmart}/' $<   > $@

samples/sample-sigconf.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigconf]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-authordraft.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigconf,authordraft]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-xelatex.tex: samples/sample-sigconf.tex
	cp $< $@

samples/sample-sigplan.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigplan,screen]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-sigchi.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigchi]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-sigchi-a.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigchi-a]{acmart}/' $< | \
	sed 's/begin{figure}\[h\]/begin{marginfigure}/' | \
	sed 's/end{figure}/end{marginfigure}/' | \
	sed 's/begin{table}/begin{margintable}/' | \
	sed 's/end{table}/end{margintable}/'   > $@


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut

distclean: clean


#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf samples/sample-*.pdf *.cls *.bst

